On Categories associated to a Quasi-Hopf algebra

A quasi-Hopf algebra $H$ can be seen as a commutative algebra $A$ in the centre $\mathcal Z(H-Mod)$ of $H-Mod$. We show that the category of $A$-modules in $\mathcal Z(H-Mod)$ is equivalent (as a monoidal category) to $H-Mod$. This can be regarded as a generalization of the structure theorem of Hopf bimodules of a Hopf algebra to the quasi-Hopf setting.

==> obrazky1/2daco2.tex <==
\begin{tikzpicture}[baseline=0.0cm]
\draw [line width=1pt] (0.0,0.0) -- (-0.18,0.08);
\draw [line width=1pt] (0.0,0.0) -- (-0.18,-0.08);
\draw [line width=1pt] (0.0,0.0) -- (-0.2,0.0);
\node at (0.0,-0.6) {{\scriptsize $A$}};
\draw [line width=1pt] (0.0,-0.4) ..controls +(0.0,0.17) and +(-0.17,0.0) .. (-0.2,0.0);
\end{tikzpicture}

